The Shape of an Image: A Study of Mapper on Images

We study the topological construction called Mapper in the context of simply connected domains, in particular on images. The Mapper construction can be considered as a generalization for contour, split, and joint trees on simply connected domains. A contour tree on an image domain assumes the height function to be a piecewise linear Morse function. This is a rather restrictive class of functions and does not allow us to explore the topology for most real world images. The Mapper construction avoids this limitation by assuming only continuity on the height function allowing this construction to robustly deal with a significant larger set of images. We provide a customized construction for Mapper on images, give a fast algorithm to compute it, and show how to simplify the Mapper structure in this case. Finally, we provide a simple procedure that guarantees the equivalence of Mapper to contour, join, and split trees on a simply connected domain.

==> proof.tex <==
\begin{comment}
\begin{theorem}
Let $\mathcal{U}$ be the covering specified in the procedure given above. Then the Mapper $M(X,f,\mathcal{U})$ is equivalent to contour tree $T(X,f)$.
\end{theorem}
\begin{proof}
Let $k<n$ and let  $
\mathcal{U}_k:=\{(c_0,d_1),(a_1,b_1),...,(c_{k-1},d_{k}),(a_{k},b_k)\}
$
. Let $X_t$ be the set $\{p\in X| f(p)\leq t \}$. We show by induction on $k$ that $M(X_{b_k},f,\mathcal{U}_k)=T(X_{b_k},f)$. For $k=1$ both It is clear that $T(X_{b_1},f)$ consists of a single node and so does  $M(X_{b_1},f,\mathcal{U}_1)$. Suppose that $M(X_{b_{k-1}},f,\mathcal{U}_{k-1})=T(X_{b_{k-1}},f)$ and we want to show $M(X_{b_k},f,\mathcal{U}_k)=T(X_{b_k},f)$. When passing from the critical point $t_{k}$ the topology of $X_{b_{k-1}}$ change according to the index of the critical point $p_k$. More precisely, when passing from the critical value $t_k$ the number of connected components of $f^{-1}(b_{k-1})$ and $f^{-1}(b_{k})$ changes. The number of connected components for the interval $f^{-1}(a_{k-1},b_{k-1})$ is the same as the number of connected component of $f^{-1}(b_{k-1})$. This is also true for $f^{-1}(a_{k},b_{k})$ is the same as the number of connected component of $f^{-1}(b_{k-1})$.


%Suppose that the number of connected components in $f^{-1}(b_{k})$ associated to the critical point $p_k$ is $l_1$ and the number of connected components in $f^{-1}(b_{k-1})$ associated to $p_k$ is $l_2$. That is there are $l_1$ edges coming to node $p_k$ and $l_2$ leaves.

\end{proof}
\end{comment}



